Human-in-the-Loop Optimization for Deep Stimulus Encoding in Visual Prostheses

Neuroprostheses show potential in restoring lost sensory function and enhancing human capabilities, but the sensations produced by current devices often seem unnatural or distorted. Exact placement of implants and differences in individual perception lead to significant variations in stimulus response, making personalized stimulus optimization a key challenge. Bayesian optimization could be used to optimize patient-specific stimulation parameters with limited noisy observations, but is not feasible for high-dimensional stimuli. Alternatively, deep learning models can optimize stimulus encoding strategies, but typically assume perfect knowledge of patient-specific variations. Here we propose a novel, practically feasible approach that overcomes both of these fundamental limitations. First, a deep encoder network is trained to produce optimal stimuli for any individual patient by inverting a forward model mapping electrical stimuli to visual percepts. Second, a preferential Bayesian optimization strategy utilizes this encoder to optimize patient-specific parameters for a new patient, using a minimal number of pairwise comparisons between candidate stimuli. We demonstrate the viability of this approach on a novel, state-of-the-art visual prosthesis model. We show that our approach quickly learns a personalized stimulus encoder, leads to dramatic improvements in the quality of restored vision, and is robust to noisy patient feedback and misspecifications in the underlying forward model. Overall, our results suggest that combining the strengths of deep learning and Bayesian optimization could significantly improve the perceptual experience of patients fitted with visual prostheses and may prove a viable solution for a range of neuroprosthetic technologies.

==> rebuttal.tex <==
\section{Rebuttal}

Reviewer YFQD:
Weaknesses: 
•	The main weakness of this paper lies in its limited novelty, as the proposed approach is merely a combination of the state-of-the-art of forward models and sample-efficient Bayesian optimization to optimally find personalized stimuli. 
•	Although this paper improvises the techniques used in the visual prostheses domain, the overall contribution of this paper is in the application of the existing ML/DL techniques in neuroprostheses, visual prostheses in particular, thus may not advance the state-of-the-art in ML/DL community. 
\textbf{The paper was submitted to NeuriPs Primary Area: Neuroscience and cognitive science (neural coding, brain-computer interfaces). We don’t claim particular contribution to ML/DL. This is an application of ML/DL to brain-computer interfaces. }
•	Though the paper reads well in many parts, it demands significant knowledge/domain expertise in visual prosthesis for a thorough understanding of the paper. 
•	Authors have missed defining/describing a few important mathematical quantities or parameters that break the flow of understanding and also raise questions about its reproducibility (Please refer to the Questions section).
•	The details provided in Section 4 give the impression that the proposed framework is tightly coupled with the problems in visual prostheses. 
•	The authors have discussed a few experimental settings in Section 4 that are apt to discuss in Section 5, though they do not contribute to the proposed method.
•	The visualization schemes used to show the empirical results do not effectively demonstrate the superiority of the proposed approach. Also, the authors do not discuss in brief the trends and the possible reasons behind them.


Questions

Figure 3: Why there is an increasing (or decreasing) trend in loss (or accuracy) plot during the initial phase of the optimization?
\textbf{This is a common pattern seen in preferential Bayesian optimization (see e.g. figure 5 in Gonzalez et al, 2017). This is due to the fact that the estimate of the maximum is $\operatorname{argmax} \mathbb{E}[g|\mathcal{D}]$. PBO is different compared to other optimization methods based on noise-free objective function evaluation where the maximum is taken over the previously sampled points. Here, the estimate of the optimum rapidly changes in the initial phase of the optimization (It is not guaranteed to improve), which explains why after observing a few data points, the estimate of the optimum can get worse.  }

Line 198: Why do authors considered only 10 simulated patients for transfer learning? is that not sparse?
\textbf{In a real-life scenario (like a clinical trial), we would initially have access to a very limited number of patients. Also, increasing the number of patients used for transfer learning would make the problem easier. The fact that our approach worked by transferring information from only a very limited set of 10 patients suggests it is very efficient. }

Line 302: Could Batch-BO strategies further reduce the latency and thus provide a quicker solution by parallelizing the data acquisition?
\textbf{Batch-PBO is indeed a possibility in this setting. However, this would significantly increase the cognitive burden for patients, as stimuli are presented sequentially. Patients would have to remember a batch of stimuli before making a comparison.  So comparisons could become even more noisy.}

Limitations: 
•	The optimization performance of PBO crucially depends on the _ generalization performance of the inherent GP surrogate model_. Authors reduce latency by avoiding online inference and instead use a transfer learning strategy. However, the source considered in the adopted transfer learning uses sparse data generated from 10 patients, thus, raising concerns about the optimality of kernel parameters and generalizability of the GP surrogates.
\textbf{Optimizing hyperparameters in the initial phase of the optimization process  with limited data, could lead to noisy and inaccurate estimates. This problem is extensively discussed in \cite{brochu_bayesian_2010}. 
It is common in BO experiments to keep the hyperparameters constant (see e.g. 
%\citep{brochu_bayesian_2010, ding_human-in-the-loop_2018, louie_semi-automated_2021,nielsen_perception-based_2015, kupcsik_robot-to-human_2018, tucker_atalante_2019, lorenz_efficiently_2019, zhao_optimization_2021}. 


Instead, we rely on hyperparameters learned on 10 previous patients, assuming they would be similar in new patients. In a real-life scenario, as new data are acquired on new patients, this set of patients could grow. 

One also has to consider the trade-off between the potential increase in performance with hyperparameter learning (which takes time) and the consequences of increased fatigue and attentional lapses in patients who would have to engage in longer HILO sessions. 
}
•	Although the authors discuss the empirical results, the lack of sufficient experiments and competing baselines (Beyeler et al. 2019, Granley et al. 2022) in the empirical results makes it hard to conclude the superiority of the proposed approach. (Please refer to the Questions section).

•	Sequential PBO may not be very suitable in time-critical situations, thus, more efficient strategies such as batch-BO could be of great use to reduce the possible latency in finding the optimal stimuli on-the-fly.

\textbf{See response above.}


Reviewer bw3i:

Weaknesses:

    It is not made super clear whether and how the parameters w of the encoder is being updated in the manuscript.
    The authors could have demonstrated a small amount of humans with sight to show the effectiveness of this optimization method.


Questions:
    The simulated patient has access to t, which is the target percept or ground truth. Is it realistic to assume the blind person could have access to that?
    In line 219 it’s written that the metric in equation (7) is also used to train the deep stimulus encoder (DSE). So the encoder’s parameters are getting updated in a rather conventional way as in the visual prosthesis literature. How to distinguish the contribution between the improvement of the encoder and the selection of patient-specific parameters? Could it be that the update of the encoder contribute the most? Ablation studies might be needed.




Reviewer HJZJ:
Weaknesses:
The primary weakness is the reliance on simulated data, and it is not clear that simulated patient choice or patient parameters to generate the data was sufficiently grounded in experimentally collected datasets. There is some discussion of how the ranges for the parameters were chosen in their simulated data, but nothing about the expected variability and how these parameters were determined in the first place (is it considered ground truth? were patient preferences included?). If the method is sufficiently generalizable to many populations of patients, as expected, then why not simulated patients outside of those limited ranges in Table 1? Lines 263-265 appear to suggest that their ranges of parameters are unlikely to be same as in the real world. A similar concern is for simulating patient preference, but here the authors' simulations (up to 33\% incorrect decisions from the patient) appear like a robust demonstration. 

One other weakness not discussed is the feasibility of their approach for actual human patients. Even if it only takes 3 seconds to update the GP and generate new stimuli, the patient must sit through and compare difficult to discern visual percepts for 100 duels. Is it likely the patient would persist? 
\textbf{100 duels would take 300 seconds (5 minutes), this is negligible compared to the very long training and rehabilitation process these patients must go through.   }

Does their judgement change over time? If this could be changed every so often, does the system need re-tuning for all ~100 duels at once? Additionally, humans see visual scenes with certain image statistics -- so MNIST may not be a reasonable or sufficient dataset for testing human perception on. Could this approach be extended to natural images, including color?

Questions:

i. Line 43 says <30 is too few parameters, but then the authors used only 13 dimensions of parameters? 
\textbf{Line 43 says the number of dimensions required for PBO to work is <30, not that it is too few parameters.}
ii. Line 129-130 appears to have a sentence cut off abruptly.
iii. Line 127: BO can’t optimize more than a small number of parameters -- clarify please? BO gets difficult in high dimensions, but this is true of many methods. How specifically does the DSE reduce this? 

\textbf{BO is known to be very challenging in high dimensions. In all previous applications of HILO, the number of parameters was small \citep{brochu_bayesian_2010, ding_human-in-the-loop_2018, louie_semi-automated_2021,nielsen_perception-based_2015, kupcsik_robot-to-human_2018, tucker_atalante_2019, lorenz_efficiently_2019, zhao_optimization_2021}. Without the use of the DSE, for example, if using a linear encoder instead, the number of parameters to tune would be the number of electrodes $\times$ the number of pixels in the input image, which is orders of magnitude larger than what current PBO algorithms can deal with. }

% Ding et al., 2018: exoskelettons 
% Louie et al., 2021: deep brain stimulators
% Brochu et al., 2010 :  Procedural animation design 
% Nielsen, 2015 :  hearing aids 
% Kupcsik et al. (2018)   robot-to-human object handover across a variety of randomly chosen contexts
 % Tucker et al. (2019):   Atalante lower-body exoskeleton.
 % Lorenz et al. (2019): maximize the phosphenes brightness elicited in transcranial alternating current stimulation 
 % Zhao et al. (2021) ; applied PBO to epidural spinal cord stimulation.  


iv. Clarify the issue in lines 154-158. The logic is not clear what the exact problem is and how it is solved here. 
v. If you didn’t restrict the range of parameters in Table 1 as heavily, would it still find the optimal values? E.g. if you increased the range by a factor of 2. 
vi. Line 232 first mention of Argus II, needs explanation and citation.
vii. What does it mean to outperform the true DSE? Line 289 
viii. Line 296 how does the approach fail?


